Towards grid-aware multi-period flexibility aggregation - A constrained zonotope approach

Aggregation schemes provide a means to reduce the computational complexity of power system operation by reducing the number of devices that are considered individually. This can be achieved with tools of computational geometry, where the feasible set is projected onto the decision variables of the point of interconnection. Set projection is computationally expensive, especially in the context of multi-period power system operation. This calls for efficiency improvements via structure exploitation of set representations. This paper proposes efficient flexibility aggregation via constrained zonotopes. We evaluate the performance of the proposed method on a 15-bus distribution grid with time-dependent elements for up to 96 timesteps. The results suggest that the presented method significantly improves computation times compared to classic polytope projection approaches.

==> ReviewerComments.tex <==
## Reviewer #1:

The paper proposes an aggregate flexibility characterization method based on constrained zonotopes (CZ), which allows for fast projection onto the flexibility-variable space. Computational performances are shown on 4- and 15-bus distribution systems with improved computation time. Some specific comments are as follows:

1. The paper states that the majority of the computation can be performed offline and additional constraints can be incorporated efficiently via one more H-intersection. This is not surprising as the offline step performs such operation one constraint at a time already so adding another constraints amounts to performing one more offline step. However, it is a little misleading to claim that this enables fast integration of revised forecast since in this case, the original constraint is no longer valid. Instead of adding a new constraint, we need to remove or modify an old constraint. As far as I understand, the CZ method does not support efficient removal or modification of an existing constraint, and an entire offline CZ construction needs to be repeated. The authors should clarify whether this is the case and if so, then updating the claim that the efficient update only applies to adding constraints, not changing them. In addition, the authors are also suggested to clarify that for typical DSO operation where the load/renewable forecast changes every 5/15 minutes, whether this implies the entire offline step needs to be repeated every update.

    -> To address this comment the respective section is refined to clarify the concept. 
    
        " This enables an efficient online update strategy for increasing problem sizes, as the underlying topology of the problem remains identical per time-step. We emphasize that, for dynamic use cases, the offline computation incorporates only the strictly static constraints (5)-(2), (4), (9) in X_i. The offline step itself converts X_i into an equivalent CZ_{off} , as elaborated in the previous section. This offline conversion accounts for the majority of the computational burden. During online operation the offline CZ_{off} serves as the baseline. Time-varying bounds, such as the integration of revised forecast data in (3), changing power demands or updated setpoint constraints, are integrated by adding the respective constraints via intersection to a copy of CZ_{off}. This results in a new CZ_{on} modeling the feasible set for each iteration. Because CZ_{off} deliberately omits previous forecast data, there is no need to computationally remove or modify existing constraints. This avoids a repetition of the offline step entirely. The computational efficiency of adding constraints dynamically via intersections is evaluated in Subsection V-B."
    
    It is sufficient to compute the offline step once. We show that individual constraints can be added sufficiently fast to be added during the online computation. This allows to compute a baseline set during the offline computation omitting all constraints containing forecast data. Therefore we do not need to remove constraints at a later point. During each online iteration, the forecast data can be added to a copy of the baseline set to model the current feasible set. While this slows down the online step it, the benchmarks highlight that it remains sufficiently fast as most of the computational burden can still be shifted to the offline computation. 
    
    → % To address this comment the respective section is refined to clarify the concept. First a feasible set is defined containing all static constraints which are not affected directly by renewed forecast data. This set is converted into a CZ which functions as a baseline. During each online iteration, this baseline set is first intersected with the remaining constraints containing the current forecast data and then projected. Future iterations can reuse the calculated baseline set eliminating the need for repeated offline computation. 
    
2. The numerical evaluation focuses exclusively on computation time improvement and the scalability of the CZ method. However, the paper does not compare the quality of the aggregate flexibility region characterization against existing methods. In particular,how does the method compare with the original zonotope method in terms of the accuracy? How does it compare with the true flexibility region? Without more concrete and quantitative results, it is hard to evaluate the effectiveness of the method.
    
    → Section III-B already states that zonotopes are limited to model centrally symmetric convex polytopes. This does not hold in general for the underlying feasible set, therefore limiting the quality of the aggregate flexibility region in contrast to polytopic sets itself. The presented method is shown to be equivalent in representational accuracy to the polytope projection in Section V-B 
    
        "The FOR modeled as CZ F^{LDF−LL}_CZ is equivalent to the respective FOR modeled as polytope F^{LDF−LL}"
    
    as long as the used variable bounds for the setup of the Bounding Zonotope meet the condition in (16). We added a reference to a previous paper [1], which already addresses the approximation accuracy and the limitations of the polytope based approach to the true non-convex flexibililty. 
    
        "For a comparison of the approximation quality of F^{LDF-LL} with the true flexibility region we refer to [19]."
    
    [19] M. Beraldo Bandeira, T. Faulwasser, and A. Engelmann, “An ADP framework for flexibility and cost aggregation: Guarantees and open problems,” Electr. Power Syst. Res., vol. 234, 2024, Art. no. 110818.
    
3. The authors are also advised to comment on the comparison with optimization-based flexibility characterization methods, such as [R1]-[R4].
    
    → To adress this commments the respective section in the introduction is extended to cover these optimization-based methods. All these methods perform inner approximations of the true feasible region based on convex / polytopic sets. The approach in [R1] is limited due to the geometry of the used inner-box approximation. Same holds for the used ellipsoidal shape in [R2],[R3]. The virtual battery model in [R4] only achieves $80\%$ of cost efficiency compared to the original polytopic set. %All of the above approaches are therefore limited in their representational accuracy compared to the underlying baseline of convex polytopic sets.
    All of the above approaches compute approximations of the aggregated flexibility area, which is not the focus of this work. Instead, this paper aims to compute the exact convex aggregated flexibility in a fast and efficient manner.
    
4. The conclusion is somewhat misleading. The authors claim "The paper addresses the central computational bottleneck arising in ADP", however, first, the paper is not about ADP and claiming projection to be a central bottleneck in ADP is an overstatement, second, projection efficiency is already established for the original zonotope method in [13]. The proposed CZ method for flexibility characterization does not change the complexity of the projection but, as the authors mentioned, provide the ability to represent non-symmetric polytopes more accurately. However, the paper does not demonstrate any evidence for accuracy improvement over the original zonotope method, nor does it compare with other methods, as I mentioned above. In summary, the authors should clearly articulate what CZ contributes over existing literature including classical zonotope method and optimization-based methods, and provide numerical evidence that corroborates such claims.
    
    → The reviewer is correct that the remaining ADP mentions were misleading and are removed. By adressing the second comment of the reviewer the benefit of the presented method in terms of accuracy improvement in contrast to zonotope approaches by achieving equivalent accuracy as polytope based approaches are emphasized. The conclusion is modified to clearly state this contribution.
    

[R1] X. Chen, E. Dall'Anese, C. Zhao, and N. Li, "Aggregate power flexibility in unbalanced distribution systems," IEEE Trans. Smart Grid, vol. 11, no. 1, pp. 258-269, Jan. 2020.

→ Consideres unbalanced distribution systems, approximation of the exact feasible region of the net power injection at the substation with an inner-box region and the upper and lower operational trajectories are defined to specify the aggregate flexibility over time. Considers network constraints. Only considers active power.

[R2] X. Chen and N. Li, "Leveraging two-stage adaptive robust optimization for power flexibility aggregation," IEEE Trans. Smart Grid, vol. 12, no. 5, pp. 3954-3965, Sep. 2021.

→ Adaptive robust optimization (ARO), considers multi-period power flexibility with network constraints and unbalanced power flow model. Considers individual active / reactive power and combined. Elliptical feasible regions of the aggreagte PQ domain. 

[R3] B. Cui, A. Zamzam, and A. Bernstein, "Network-cognizant time-coupled aggregate flexibility of distribution systems under uncertainties," IEEE Control Syst. Lett., vol. 5, no. 5, pp. 1723-1728, Nov. 2021.

→ Adjustable robust optimization to compute the maximum volume inscribed ellipsoid for the projection of the active power of distribution system flexibility region at a substation at different times. Based on a linear model resulting in a polytopic initial set. Consideres network awareness, load uncertainty, and time coupling. Results only compared to hyper cube based approach, while outperforming that approach still limited accuracy due to ellipsoidal shape. Tested on grid with 126 multiphase nodes and 4 timesteps.

[R4] Z. Tan, A. Yu, H. Zhong, X. Zhang, Q. Xia, and C. Kang, "Optimal virtual battery model for aggregating storage-like resources with network constraints," CSEE J. Power Energy Syst., vol. 10, no. 4, pp. 1843-1847, Jul. 2024.

→ Optimiization based virtual battery model for linearized DistFlow, says calculating exact projection infeasible for 13 buses and 5 hour receeding horizon, instead inner approximation with adjustable robust optimization (ARO) to ensure disaggregation feasibilty. Utillizes Bender Decomposition. Considers grid constraints however for the given testcase only around $80\%$ of cost efficiency as optimization of linearized DistFlow without aggregation. Highlights limitation of inner approximation.

## Reviewer 2:

The paper proposes using constrained zonotopes to accelerate the computation of multi-period feasible operating regions arising in distribution grid OPF problems. The goal is to reduce the computational bottleneck associated with set projection for hierarchical TSO-DSO coordination.

The topic is relevant, and the idea of leveraging CZs for multi-period flexibility aggregation is promising. I have the following comments:

1. The contributions should be more clearly stated. From different parts of the introduction, the authors imply considering some features, e.g., multiple connections between DSO and TSO, variable reference voltage, time-dependent elements, active-reactive spaces, and more importantly computational performance improvement. The paper would benefit from a summary of claimed novelties at the end of the introduction. 
    
    → To adress this comment, the respective paragraph in the introduction is modified to clearly state the contribution of extending the non-iterative projection-based formulation to compute voltage dependent FORs to a multi-period setting with time-dependent elements.
    
2. There are several notational and mathematical issues:
    1. ADP is never introduced  
        
        → We thank the reviewer for pointing it out, we have removed the mentions of ADP.
        
    2. Notation in Eq. (1) and surrounding text is unclear. Several symbols (sets, indexing, variables) appear before proper definition. 
        
        → The surrounding text is modified to proper define the symbols and Eq. (1) is adjusted.
        
    3. Eq. (4) is inconsistent / incorrect. The parameter α is treated as a power factor angle in the first constraint, but as tangent of the angle in the second constraint. 
        
        → Thanks to the comment, the corresponding equations were clarified and corrected.
        
    4. The Jacobian-vector product is dimensionally inconsistent. A transpose is missing. 
        
        → The equation was formatted incorrectly, the transpose is now at the correct place.
        
    5. In the definition of the CZ, = should be replaced with <= 
        
        → The definition of the CZ is correct with "=", as the constraints on the internal factors are equality constraints. For future details the reviewer is refereed to [19].
        
        [19] J. K. Scott, D. M. Raimondo, G. R. Marseglia, and R. D.
        Braatz, “Constrained zonotopes: A new tool for set-based estimation and fault detection,” Automatica, vol. 69, pp. 126–136,
        2016.
        
    6. In power flow formulation in (8), p_{m,l} and q_{m,l} should be values at t0. Right now, they seem to be variables and the resulting (6) is still non-linear. 
        
        → The authors thank the reviewer to point out this clear mistake.
        
3. The DistFlow equations (5)-(8) are linearized around a fixed point t0. How did authors consider local linearization for the whole feasible region? What is the role of t0? 
    
    → The respective paragraph is revised in order to address this comment. Additionally a previous paper is referenced in which the local linearization is evaluated with respect to it's accuracy with the common approach of neglecting line impedances. 
    
4. The manuscript states "we consider LinDistFlow with and without loss linearization as discussed in Section II." However, section II contains no such discussion and no numerical comparison is provided. This must be clarified and supported with results.
    
    → This statement is in fact misleading as the evaluation only considers LinDistFlow with loss linearization as it was shown to be a more accurate convex approximation of the true FOR in a previous paper [1]. Section II is modified to elaborate the difference between both formulations but the above mentioned statement is removed from section V. 
    
    [1] M. Beraldo Bandeira, T. Faulwasser, and A. Engelmann, “An ADP framework for flexibility and cost aggregation: Guarantees and open problems,” Electr. Power Syst. Res., vol. 234, 2024, Art. no. 110818.
    
5. The authors refer to the 15-bus test feeder as "medium-sized" or "large-scale." However, 15 buses is very small for MV networks of interest in this paper. Also, only four nodes contain DERs and the feeder is almost entirely passive. How, does the proposed method scale with larger networks and more DER integration?
    
    → The reviewer is correct that the 15-bus test feeder is quiet small. However, the problem size increases significantly with time-horizon length. This results in a medium-sized to large-scale problem depending on the problem size and given the fact that we consider time dependent elements. To emphasize this, section V-B is adapted and a figure showcasing the scaling of the problem with time horizon length is added.
    
6. Benchmarking is incomplete
    
    → Given no further details not addressable directly, hopefully remaining changes resolve this comment.
    
7. The proposed method is used as time-ahead decision support. This require considering load and generation uncertainty. 
    
    → This is object of future research as this method enables the time-ahead decision support in the first place. Future research will address the consideration of uncertainties in the proposed framework. This direction of future research is added to the outlook.
    
8. "rm,l and xm,l are, respectively, the line reactance and capacitance" this should be resistance and reactance?
    
    → The authors thank the reviewer to point out this clear mistake.
    
9. the charging and discharging efficiency of the battery is not considered, however, this is a crucial omission in the proposed model as this consideration in important. Its omission of course helps in storage charge evolution to be denoted by simple linear equation in eq. 12, which may not be realistic. Consider storage efficiencies can be as low as $80\%$ for grid scale batteries (decreasing even further with aging of batteries), it should be considered.
    
    → For the purpose of this paper a simple battery model is considered as the battery dynamics are no object of research here, however, in future research more accurate models should be incorporated. This direction of future research is added to the outlook.
    

## Reviewer #3:

The paper considers a TSO-DSO coordination problem in which, due to privacy concerns among other factors, DSO data cannot be shared with the TSO. To address this, earlier work has proposed replacing the original detailed grid feasible sets with their projections onto the space of shared variables between DSOs and TSOs, corresponding to the interconnection points.

The paper essentially considers this projection problem and proposes to use earlier work on 'constrained zonotopes' [1] - work commented below in see 2. - as a way to efficiently handle the projection problem, since projections of polytopes described as the intersection of half-spaces (H-rep) is notably difficult and intractable for high dimensional polytopes, while manageable when working with 'constrained zonotope representations'.

While the work is interesting and well written, a substantial part of it is a direct application of [1] to a TSO-DSO coordination context. There are, moreover, two main concerns, and responses from the authors would be welcome to provide any necessary clarifications.

1. First, it seems that the 'constrained zonotope' representation using elements of [1] doesn't necessarily resolve the constraint privacy challenge of the DSO, given that even after projection of the 'constrained zonotope representation of the initial feasible set', key information if not all the information on the initial linear constraints Hx<= k of the DSOs remain somewhat visible in the constrained zonotope data corresponding to the projection. Indeed, using notation in [1] (which is the basis of the present paper), the constraints Hx<= k are somehow 'reproduced' (wording of [1]) in the constraints of the initial feasible set's constrained zonotope representation, roughly just multiplied there by G (more precision in [1]), the generator of the enclosing zonotope (which is then further cut/refined by adding back these Hx<=k constraints defining the convex polytope being represented as a CG). Since G, c, HG, k, ..., are known, and given that G as defined in 16b of the present paper is invertible (generator of an enclosing box), it seems that key or all the information on Hx<=k can be retrieved from the representation of the projection given in (21)… despite the initial goal being to share a projected set discarding private DSO data. Such a problem would not occur with H-rep projections of H-rep polytopes representing grid constraints. Please discuss and provide clarifications addressing this point.
    
    → To address this comment section III is extended to clarify the privacy concerns. In contrast to polytope projection which implicitly obscures sub-grid details this is not the case for the proposed CZ method. As the reviewer correctly points out, without additional steps, the DSO's information may be retrieved from the internal constraints of the communicated projected CZ. However, the proposed method allows a clear separation between online and offline communication where the offline computation determines the equivalent CZ representation for the convex feasible set. The offline step allows seamless integration of additional privacy-preserving transformations masking critical information without affecting accuracy of the communicated projection.
    
2. The points made in [1] about the simplicity of certain set operations like projections when using constrained zonotope representations of convex polytopes seem somewhat trivial and potentially misleading. The apparent ease of projection in the constrained-zonotope framework, as opposed to the challenges with H-rep, follows from three facts:
    
    (a) zonotopes defined as linear images of hypercubes (equivalent to the def. as Minkowski sums of line segments)
    
    (b) projecting such linear images amounts to composing linear maps, which remains straightforward to express in matrix form, and
    
    (c) the "constrained" part essentially reproduces the half-space constraints of the original polytope within the constrained-zonotope representation, as described in [1].
    
    (d) Finally, the 'zonotope' component is basically about an enclosing box and working with linear map representations.
    
    Responses to the concerns outlined above, or indications of any misunderstandings, along with corresponding clarifications in the paper, would be helpful. Otherwise, the paper is clear and well written.
    
    → I don’t quite grasp the question or concern behind the comment. The stated aspects enable the proposed method which combines the approximation accuracy of polytopes with the fast projection via linear map of zonotopes.
    
    [1] Scott, Joseph K., et al. "Constrained zonotopes: A new tool for set-based estimation and fault detection." Automatica 69 (2016): 126-136.

==> flow_cz_appr.tex <==
% \documentclass{standalone}
% \usepackage{tikz}
% \usetikzlibrary{positioning}
% \begin{document}

    \begin{tikzpicture}[
  every node/.style = {draw, rectangle, rounded corners, align=center, 
    minimum height=1cm,
    minimum width=10cm},
  edge from parent/.style = {draw, -latex, -}]

    \begin{scope}[every node/.style = {draw, rectangle, rounded corners, align=center, 
    minimum height=1cm,
    minimum width=10cm}]
        \node[fill=lightgray!20] (FeasibleSet) at (0,0) {Feasible set of MS-OPF based on LDF-LL formulation};
        \node[below=0.5 of FeasibleSet,fill=lightgray!50] (BZ) {Bounding Zonotope};
        \node[below=0.5 of BZ,fill=titlegreen] (CZ) {Constrained Zonotope};
    \end{scope}

    %\draw[-latex,line width=2pt] (FeasibleSet)--(BZ) node[midway,right, draw=none] (proj_poly){};
  % \node[below left=0.8 and 1.9 of ConSysSta.south, anchor=north] (EleMacSta) {Electric Machine\\Stability};
  % \node[below right=0.8 and 1.9 of ConSysSta.south, anchor=north] (ConSta) {Converter\\Stability};

  % \node[below left=0.8 and 1.9 of BalSta.south, anchor=north] (VolSta) {Voltage\\Stability};
  % \node[below right=0.8 and 1.9 of BalSta.south, anchor=north] (FreSta) {Frequency\\Stability};
  
  % \node[below=0.8 of VolSta] (SmaDisR) {Small\\Disturbance};
  % \node[below=0.8 of FreSta] (LarDisR) {Large\\Disturbance};
  % \node[below=0.8 of SmaDisR] (ShoTerR) {Short Term};
  % \node[below=0.8 of LarDisR] (LonTerR) {Long Term};

  % \node[below=0.8 of EleMacSta] (SmaDisL) {Small\\Disturbance};
  % \node[below=0.8 of ConSta] (LarDisL) {Large\\Disturbance};
  % \node[below=0.8 of SmaDisL] (ShoTerL) {Short Term};
  % \node[below=0.8 of LarDisL] (LonTerL) {Long Term};

  %   % First Level
    \draw[-latex] (FeasibleSet.south)-| (BZ.north);
    \draw[-latex] (BZ.south)-| (CZ.north);
   %                        -| ;
  %   \draw (ConSta.north)-- ++(0,0.4)
  %                       -- ++(-1.9,0);

  %   \draw (BalSta.south)-- ++(0,-0.4)
  %                         -| (VolSta.north);
  %   \draw (FreSta.north)-- ++(0,0.4)
  %                       -- ++(-1.9,0);
  

  %   % Left side
  %   \draw (EleMacSta.south)-- ++(0,-0.2)
  %                         -- ++(1.9,0)
  %                         -- ++(0,-0.4)
  %                         -| (SmaDisL.north);
  %   \draw (ConSta.south)-- ++(0,-0.2)
  %                       -- ++(-1.9,0);
  %   \draw (LarDisL.north)-- ++(0,0.2)
  %                       -- ++(-1.9,0);

  % % Right side between Disturbance and Term                        
  % \draw (SmaDisL.south)-- ++(0,-0.2)
  %                         -- ++(1.9,0)
  %                         -- ++(0,-0.4)
  %                         -- ++(-1.9,0)
  %                         -- (ShoTerL.north);
  % \draw (LarDisL.south)-- ++(0,-0.2)
  %                         -- ++(-1.9,0);
  % \draw (LonTerL.north)-- ++(0,0.2)
  %                         -- ++(-1.9,0);

  % % Left side
  % \draw (VolSta.south)-- ++(0,-0.2)
  %                         -- ++(1.9,0)
  %                         -- ++(0,-0.4)
  %                         -- ++(-1.9,0)
  %                         -- (SmaDisR.north);
  % \draw (FreSta.south)-- ++(0,-0.2)
  %                         -- ++(-1.9,0);
  % \draw (LarDisR.north)-- ++(0,0.2)
  %                         -- ++(-1.9,0);

  % % Left side between Disturbance and Term                        
  % \draw (SmaDisR.south)-- ++(0,-0.2)
  %                         -- ++(1.9,0)
  %                         -- ++(0,-0.4)
  %                         -- ++(-1.9,0)
  %                         -- (ShoTerR.north);
  % \draw (LarDisR.south)-- ++(0,-0.2)
  %                         -- ++(-1.9,0);
  % \draw (LonTerR.north)-- ++(0,0.2)
  %                         -- ++(-1.9,0);
                          

\end{tikzpicture}

% \end{document}

